Post-mortem on a deep learning contest: a Simpson's paradox and the complementary roles of scale metrics versus shape metrics

To understand better good generalization performance in state-of-the-art neural network (NN) models, and in particular the success of the ALPHAHAT metric based on Heavy-Tailed Self-Regularization (HT-SR) theory, we analyze of a corpus of models that was made publicly-available for a contest to predict the generalization accuracy of NNs. These models include a wide range of qualities and were trained with a range of architectures and regularization hyperparameters. We break ALPHAHAT into its two subcomponent metrics: a scale-based metric; and a shape-based metric. We identify what amounts to a Simpson's paradox: where "scale" metrics (from traditional statistical learning theory) perform well in aggregate, but can perform poorly on subpartitions of the data of a given depth, when regularization hyperparameters are varied; and where "shape" metrics (from HT-SR theory) perform well on each subpartition of the data, when hyperparameters are varied for models of a given depth, but can perform poorly overall when models with varying depths are aggregated. Our results highlight the subtlety of comparing models when both architectures and hyperparameters are varied; the complementary role of implicit scale versus implicit shape parameters in understanding NN model quality; and the need to go beyond one-size-fits-all metrics based on upper bounds from generalization theory to describe the performance of NN models. Our results also clarify further why the ALPHAHAT metric from HT-SR theory works so well at predicting generalization across a broad range of CV and NLP models.

==> table4-fin.tex <==

\begin{tabular}{|p{1.05in}|c|c|c|c|c|c|c|c|c|c|}
\hline
& \multicolumn{2}{|c|}{ \SPECTRALNORM      } 
& \multicolumn{2}{|c|}{ \FROBENIUSNORM     } 
& \multicolumn{2}{|c|}{ \ALPHA             } 
& \multicolumn{2}{|c|}{ \QUALITYOFALPHAFIT } 
\\
\hline
               &  $R^2$ & Kendall-$\tau$ &  $R^2$ & Kendall-$\tau$ &  $R^2$ & Kendall-$\tau$ &  $R^2$ & Kendall-$\tau$  \\
\hline
\TASKONE - 0xx & 0.34  &  0.41  & 0.00  &  -0.03  &\textbf{ 0.55 } & \textbf{ -0.55 } & 0.02  &  -0.10  \\
\hline
\TASKONE - 1xx & 0.68  & \textbf{ 0.73 } & 0.29  &  -0.30  &\textbf{ 0.88 } &  -0.48  & 0.00  &  0.15  \\
\hline
\TASKONE - 2xx & 0.59  &  0.73  & 0.42  &  0.55  &\textbf{ 0.69 } &  -0.52  & 0.67  & \textbf{ -0.82 } \\
\hline
\TASKONE - 5xx &\textbf{ 0.58 } & \textbf{ 0.60 } & 0.19  &  -0.25  & 0.09  &  -0.10  & 0.04  &  0.18  \\
\hline
\TASKONE - 6xx & 0.22  & \textbf{ 0.59 } & 0.05  &  -0.10  &\textbf{ 0.67 } &  -0.32  & 0.10  &  -0.13  \\
\hline
\TASKONE - 7xx & 0.58  & \textbf{ 0.61 } & 0.38  &  0.58  & 0.45  &  -0.51  &\textbf{ 0.60 } &  -0.58  \\
\hline
\TASKONE - AVG & 0.50  & \textbf{ 0.61 } & 0.22  &  0.07  &\textbf{ 0.55 } &  -0.41  & 0.24  &  -0.22  \\
\hline
\hline
\TASKTWO - 2xx & 0.05  &  0.01  & 0.67  & \textbf{ -0.84 } & 0.69  &  -0.74  &\textbf{ 0.89 } &  -0.83  \\
\hline
\TASKTWO - 10xx & 0.32  &  0.60  & 0.60  &  -0.53  & 0.62  & \textbf{ -0.67 } &\textbf{ 0.70 } &  -0.67  \\
\hline
\TASKTWO - 6xx & 0.21  & \textbf{ 0.36 } & 0.01  &  -0.05  &\textbf{ 0.36 } &  -0.25  & 0.35  &  -0.25  \\
\hline
\TASKTWO - 9xx & 0.17  &  0.47  & 0.65  & \textbf{ -0.87 } & 0.64  &  \textbf{-0.87}  &\textbf{ 0.91 } &  \textbf{-0.87}  \\
\hline
\TASKTWO - AVG & 0.19  &  0.36  & 0.48  &  -0.57  & 0.58  &  -0.63  &\textbf{ 0.71 } & \textbf{ -0.66 } \\
\hline
\end{tabular}


==> table5-fin.tex <==

%
\begin{tabular}{|p{0.85in}|c|c|c|c|c|c|c|c|c|c|}
\hline
& \multicolumn{2}{|c|}{ \ALPHAHAT      } 
& \multicolumn{2}{|c|}{ \DISTANCEFROMINIT     } 
& \multicolumn{2}{|c|}{ \SHARPNESS             } 
& \multicolumn{2}{|c|}{ \SVDSMOOTHING } 
\\
\hline
               &  $R^2$ & Kendall-$\tau$ &  $R^2$ & Kendall-$\tau$ &  $R^2$ & Kendall-$\tau$ &  $R^2$ & Kendall-$\tau$  \\
\hline

Task1 - 0xx &  \textbf{0.55} & -0.55 & 0.47 &  \textbf{0.7}4 & 0.26 & 0.72 & 0.53 & 0.61 \\
Task1 - 1xx &  \textbf{0.88} & -0.48 & 0.58 &  \textbf{0.85} & 0.43 & 0.82 & 0.75 & 0.79 \\
Task1 - 2xx & 0.69 & -0.52 & 0.32 & 0.61 & 0.30 & 0.48 &  \textbf{ 0.84} &  \textbf{0.76} \\
Task1 - 5xx & 0.09 & -0.10 & 0.60 & 0.77 &  \textbf{0.63} &  \textbf{0.76} & 0.38 & 0.43 \\
Task1 - 6xx &  \textbf{0.61} & -0.37 & 0.52 & 0.73 & 0.59 &  \textbf{0.76} & 0.40 & 0.45 \\
Task1 - 7xx & 0.45 & -0.51 & 0.28 & 0.61 & 0.54 & 0.64 &  \textbf{0.67} &  \textbf{0.67} \\
Task1 - AVG & 0.55 & -0.42 & 0.46 & \textbf{0.72} & 0.46 & 0.70 &  \textbf{0.60} & 0.62 \\
\hline\hline

Task2 - 2xx  & 0.69 & -0.74 & 0.22 & 0.49 & 0.34 & 0.75 &  \textbf{0.95} &  \textbf{0.83} \\
Task2 - 6xx  &  \textbf{0.36} & -0.25 & 0.21 & 0.37 & 0.22 &  \textbf{0.39} & 0.27 & 0.27 \\
Task2 - 9xx  & 0.64 &  \textbf{-0.87} & 0.49 & 0.60 & 0.39 & 0.73 &  \textbf{0.71} &  \textbf{0.87} \\
Task2 - 10xx & 0.65 & -0.70 & 0.41 &  \textbf{0.73} & 0.41 & 0.68 &  \textbf{0.68} &  \textbf{0.73} \\
Task2 - AVG  & 0.58 & -0.64 & 0.33 & 0.55 & 0.34 & 0.64 &  \textbf{0.65} &  \textbf{0.67} \\
\hline
\end{tabular}

